Probabilistic Programming with Exact Conditions

We spell out the paradigm of exact conditioning as an intuitive and powerful way of conditioning on observations in probabilistic programs. This is contrasted with likelihood-based scoring known from languages such as Stan. We study exact conditioning in the cases of discrete and Gaussian probability, presenting prototypical languages for each case and giving semantics to them. We make use of categorical probability (namely Markov and CD categories) to give a general account of exact conditioning which avoids limits and measure theory, instead focusing on restructuring dataflow and program equations. The correspondence between such categories and a class of programming languages is made precise by defining the internal language of a CD category.

==> equational_presentation.tex <==

\section{Equational Presentation of the Gaussian Language}
\label{sec:equational_theory}

We make use of $\cond(\gauss)$ to give denotational semantics to our Gaussian language from \Cref{sec:gaussian_language} and show this semantics is fully abstract (\Cref{prop:full_abstraction}). The result of this section is then dedicated to understanding $\cond(\gauss)$ in more detail, by deriving an equational presentation and normal forms.

\subsection{Denotational Semantics}
\label{sec:denotational}

The Gaussian language embeds into the internal language of $\cond(\gauss)$, where $x \eq y$ is translated as $(x - y) \eqo 0$ as in \Cref{sec:cond_on_equality}. A term $\vec x : R^m \vdash e : R^n$ denotes a conditioning channel $\sem{e} : m \obsto n$.

\begin{proposition}[Correctness]
	If $(e,\psi) \red (e',\psi')$ then $\sem{e}\psi = \sem{e'}\psi'$. If $(e,\psi) \red \bot$ then $\sem{e} = \bot$.
\end{proposition}
\begin{proof}
	We can faithfully interpret $\psi$ as a state in both $\gauss$ and $\cond(\gauss)$. If $x \vdash e$ and $(e,\psi) \red (e',\psi')$ then $e'$ has potentially allocated some fresh latent variables $x'$. We show that
	\begin{equation}
	\letin{x}{\psi} (x,\sem{e}) = \letin{(x,x')}{\psi'} (x,\sem{e'}).
	\end{equation}
	This notion is stable under reduction contexts. 
	
	Let $C$ be a reduction context. 
	Then
	\begin{align*}
	&\letin x \psi (x,\sem{C[e]}(x)) \\
	&= \letin x \psi \letin y {\sem{e}(x)} (x,\sem{C}(x,y)) \\
	&= \letin {(x,x')} {\psi'} \letin y {\sem{e'}(x,x')} (x,\sem{C}(x,y)) \\
	&= \letin {(x,x')} {\psi'} (x,\sem{C[e']})
	\end{align*}
	Now for the redexes
	\begin{enumerate}
		\item The rules for $\mathrm{let}$ follow from the general axioms of value substitution in the internal language
		\item For $\normal()$ we have $(\normal(), \psi) \red (x',\psi \otimes \mathcal N(0,1))$ and verify
		\begin{align*}
		&\letin x \psi (x,\sem{\normal()}) \\
		&= \psi \otimes \mathcal N(0,1) \\
		&= \letin {(x,x')} {\psi \otimes \mathcal N(0,1)} (x,\sem{x'})
		\end{align*}
		\item For conditioning, we have $(v\eq w,\psi) \red ((), \psi|_{v=w})$. We need to show
		\begin{align*}
		&\letin x \psi (x, \sem{v \eq w}) = \letin x {\psi|_{v=w}} (x,())
		\end{align*}
		Let $h=v-w$, then we need to the following morphisms are equivalent in $\cond(\gauss)$:
		\[ \input{conditioning/cond_exact.tikz} \]
		Applying \Cref{prop:closedterms} to the left-hand side requires us to compute the conditional $\langle \id, h\rangle\psi|_2 \circ 0$, which is exactly how $\psi|_{h=0}$ is defined.
	\end{enumerate}
	\vspace{-12pt}
\end{proof}

\begin{theorem}[Full abstraction]
	\label{prop:full_abstraction}
	$\sem{e_1} = \sem{e_2}$ if and only if $e_1 \approx e_2$ (where $\approx$ is contextual equivalence, \Cref{def:ctxequiv}).
\end{theorem}
\begin{proof}
	For $\Rightarrow$, let $K[-]$ be a closed context. Because $\sem{-}$ is compositional, we obtain $\sem{K[e_1]} = \sem{K[e_2]}$. If both succeed, we have reductions $(K[e_i], !) \red^* (v_i,\psi_i)$ and by correctness $v_1\psi_1 = \sem{K[e_1]} = \sem{K[e_2]} = v_2\psi_2$ as desired. If $\sem{K[e_1]} = \sem{K[e_2]} = \bot$ then both $(K[e_i], !) \red^* \bot$. 
	
	For $\Leftarrow$, we note that $\cond$ quotients by contextual equivalence, but all Gaussian contexts are definable in the language. 
\end{proof}

\subsection{Equational Theory}\label{sec:equational_theory_axioms}

\newcommand{\ajname}{\mathrel{\vdash\!\!\!_{\mathsf{a}}}}
\newcommand{\cjname}{\mathrel{\vdash\!\!\!_{\mathsf{c}}}}
\newcommand{\aj}[3]{#1\ajname #2:#3}
\newcommand{\cj}[3]{#1\cjname #2:#3}
\newcommand{\realtype}{\rv}
\newcommand{\abort}\bot
\newcommand{\returnname}{\mathrm{return}}
\newcommand{\returnalg}[1]{\returnname(#1)}
\newcommand{\nor}[2]{\nu #1.#2}

We now give an explicit presentation of the equality between programs in the Gaussian language in the style of \Cref{sec:algebraic-Bernoulli}. We demonstrate the strength of the axioms by using them to characterize normal forms for various fragments of the language (\Cref{sec:gauss_nf}). Besides an axiomatization of program equality, this can also be regarded in other equivalent ways, such as a presentation of a PROP by generators and relations \citep{discussion:props}, or as a presentation of a strong monad by algebraic effects, or as a presentation of a Freyd category (\Cref{bg:second_order}). But we approach from the programming language perspective. \\

Similarly to the shorthand for Beta-Bernoulli (\Cref{sec:beta_alg}), we transform the Gaussian language into an algebraic form that fits the framework of second-order algebra (\Cref{bg:second_order}). The reader may find it helpful to think of this as a normal form for the language modulo associativity of `let'. We begin by considering a fragment of the language with the following modifications: only variables of type $\realtype$ are allowed in the typing context~$\Gamma$; we have an explicit command for failure~($\bot$); we separate the typing judgement in two: judgements for expressions of affine algebra~$\ajname$ and for general computational expressions~$\cjname$; we have an explicit coercion `$\returnname$' between them for clarity. 
\[ \infer{\aj{\Gamma,x : \realtype,\Gamma'} x \realtype}{}  
\quad\ 
\infer{\aj{\Gamma}{s+t}{\realtype}}{\aj\Gamma s\realtype \quad\aj\Gamma t \realtype}
\quad\ 
\infer{\aj\Gamma {\alpha \cdot t} \realtype}{\aj\Gamma t\realtype}
\]\[
\infer{\aj\Gamma {\underline{\beta} }\realtype}{}
\qquad
\infer{\cj\Gamma {\letin x {\normal()} t}\realtype^n }{\Gamma, x : \realtype \vdash t : \realtype^n} 
\]\[
\infer{\cj\Gamma  {(s \eq t);u} {\realtype^n}}{\aj\Gamma s \realtype \quad \aj \Gamma t \realtype\quad \cj\Gamma u {\realtype^n}}
\]
\[
\infer{\cj\Gamma {\returnalg{t_1,\dots,t_n}} {\realtype^n}}{\aj\Gamma {t_1} \realtype\quad\dots\quad \aj\Gamma {t_n} \realtype}
\qquad
\infer{\cj\Gamma \abort {\realtype^n}}{}
\]

There is no general sequencing construct, but we can combine expressions using the following substitution constructions, whose well-typedness is derivable. 
\[
\infer{\cj{\Gamma,\Gamma'} {t[s/x]}{\realtype^n} }{\cj{\Gamma,x:\realtype,\Gamma'}t {\realtype^n}\quad \aj {\Gamma,\Gamma'} s \realtype} \qquad
\infer{\cj{\Gamma} {t[x_1,\dots,x_n.u/\returnname]}{\realtype^n} }{\cj{\Gamma}t {\realtype^m}\quad \cj {\Gamma,x_1,\dots,x_m:\realtype} {u} {\realtype^n}}
\]
\newcommand{\ceq}[4]{\cj{#1}{#3 \equiv #4}{\realtype^{#2}} }
\newcommand{\ceqal}[4]{\cj{#1&}{#3 \equiv #4}{\realtype^{#2}} }
\newcommand{\retname}{\mathrm{r}}
\newcommand{\ret}[1]{\retname[#1]}
In the second form we replace the return statement of an expression with another expression, capturing variables appropriately. The precise definition of this hereditary substitution is standard in logical frameworks (e.g.~\citep{adams-tf}, \citep{staton:predicate_logic}), for example:
\begin{multline*}
\hspace{-3mm}\big(\letin x {\normal()} {\returnalg{x+3}}
\big)[(a.a\eq 4;\returnalg a)/\returnname]\\
=\ \letin x {\normal()} {(x+3)\eq 4;\returnalg{x+3}}\end{multline*}
For brevity, we introduce shorthands $\nor x t$ for $\letin x {\normal()} t$, $\retname$ for $\returnname$ and drop `$;$' when unambiguous. Now the syntax matches the formalism of a second-order algebraic theory (\Cref{bg:second_order}) of the signature
\[ \nu : (0 \s 1) \qquad \bot : (0 \s -) \qquad (\eq) : (2 \s 0) \]
Note that $\retname$ is really the name of a unique suitably typed metavariable. Because the signature has no operation taking more than one computation, no more than one metavariable is necessary.

The theory is parameterized over an underlying theory of values, which is affine algebra: The type $\realtype$ has the structure of a \emph{pointed vector space}, which obeys the usual axioms of vector spaces plus constant symbols $(\underline{\beta})_{\beta \in \R}$ subject to 
\[ \alpha \cdot \underline{\beta} = \underline{\alpha\beta}, \underline{\alpha} + \underline{\beta} = \underline{\alpha + \beta} \]
Terms modulo equations are affine functions. The category theorist will recognize the category $\catname{Aff}=\gauss_\det$ as the Lawvere theory of pointed vector spaces.

We axiomatize equality by closing the following axioms under the two forms of substitution and also congruence. The following axioms characterize the conditioning-free fragment of the language, that is, Gaussian probability
\begin{align}
\ceqal {} 0 {\nor x {\ret{}}} {\ret{}} \label{ax:discard} \tag{DISC} \\
\ceqal {} n {\nor{\vec x} {\ret{U \vec x}}} {\nor {\vec x} {\ret {\vec x}}} \text{ if $U$ orthogonal} \label{ax:orth} \tag{ORTH}
\end{align}

The following are commutativity axioms for conditioning
\begin{align}
\ceqal {\hspace{-4mm}a,b,c,d }0 {(a \eq b)(c \eq d)\ret{}}{(c \eq d)(a \eq b)\ret{}} \label{ax:cond_comm} \tag{C1} \ \\ 
\ceqal{a,b }1 {(a \eq b);\nor x{\ret{x}}} {\nor x{(a \eq b)\ret{x}}}  \label{ax:nu_comm_cond} \tag{C2} \\\
\ceqal {a,b} n {(a \eq b)\bot} \bot \label{ax:fail_absorb} \tag{C3} \
\end{align}
while the following encode specific properties of $(\eq)$
\begin{align}
\ceqal a 0 {(a \eq a)\ret{}}{\ret{}} \label{ax:cond_tauto} \tag{TAUT} \ \\ 
\ceqal{}0 {(\underline{0} \eq \underline{1})\ret{}} {\bot} \label{ax:fail_incons} \tag{FAIL} \ \\
\ceqal{a,b} 1 {(a \eq b)\ret a}{(a \eq b)\ret b} \label{ax:cond_subst} \tag{SUBS} \ \\
\ceqal {}1{\nor x{(x \eq \underline c)\ret{x}}} {\ret{\underline c}} \label{ax:cond_init}  \tag{INIT}
\end{align}
Lastly, we add the special congruence scheme
\begin{align}
\ceq{\Gamma} 0 {(s \eq t)\ret {}} {(s' \eq t')\ret {}} \label{ax:cong} \tag{CONG} \
\end{align}
whenever $(s=t)$ and $(s'=t')$ are interderivable equations over $\Gamma$ in the theory of pointed vector spaces. \\

Axioms~\eqref{ax:discard} and~\eqref{ax:orth} completely axiomatize the fragment of the language without conditioning (\Cref{prop:gauss_complete}). Axioms~\eqref{ax:cond_comm}-\eqref{ax:fail_absorb} describe dataflow -- all the operations distribute over each other. The reader should focus on the remaining five axioms \eqref{ax:cond_tauto}-\eqref{ax:cong}, which are specific to conditioning. 

\subsection{Normal forms}
\label{sec:gauss_nf}

\begin{proposition}
	\label{prop:gauss_complete}
	Axioms \eqref{ax:discard}-\eqref{ax:orth} are complete for $\gauss$. That is, conditioning-free terms $\vec x : \rv^n \vdash u,v : \rv^n$ denote the same morphism in $\gauss$ if and only if $\vec x \vdash u \equiv v$ is derivable from the axioms.
\end{proposition}
\begin{proof}
	The axioms are clearly validated in $\gauss$; probability is discardable and independent standard normal Gaussians are invariant under orthogonal transformations. Note that $\nu$ commutes with itself because permutation matrices are orthogonal. 
	
	It is curious that these laws completely characterize Gaussians: Any term normalizes to the form $\nu \vec z.\ret{A \vec x + B \vec z + \vec c}$, denoting the map $(A,\vec c,BB^T)$ in $\gauss$. Consider some other term $\nu \vec w.\varphi[A'\vec x + B'\vec w + \vec c']$ that has the same denotation. By \eqref{ax:discard}, we can without loss of generality assume that $\vec z$ and $\vec w$ have the same dimension. The condition $(A,c,BB^T)=(A',c',B'(B')^T)$ implies $A=A',\vec c= \vec c'$. By \Cref{prop:orth_equivalence} there is an orthogonal matrix $U$ such that $B' = BU$. So the two terms are equated under \eqref{ax:orth}.
\end{proof}

\begin{example}
	\label{ex:alg_diagonal}
	\[ \nu x.\nu y. \ret{x+y} \equiv \nu y.\ret{\sqrt 2 \cdot y} \]
\end{example}
\begin{proof}
	Let $s=1/\sqrt 2$, then the matrix $U = \begin{pmatrix} s & s \\ -s & s \end{pmatrix}$ is orthogonal. Thus
	\begin{align*}
	\nu x.\nu y. \ret{x+y} 
	&\equiv \nu x.\nu y. \ret{(sx + sy) + (-sx + sy)} \\
	&\equiv \nu x.\nu y. \ret{\sqrt 2 y} \\
	&\equiv \nu y. \ret{\sqrt 2 y} \
	\end{align*} 
	where we apply \eqref{ax:orth}, affine algebra and \eqref{ax:discard}.
\end{proof}

We proceed to showing the consistency of the axioms for conditioning.

\begin{proposition}
	Axioms \eqref{ax:discard}-\eqref{ax:cong} are valid in $\cond(\gauss)$
\end{proposition}
\begin{proof}
	Sketch. The commutation properties are straightforward from string diagram manipulation. 
	\begin{description}
		\item[{\eqref{ax:cond_subst}}]~Write $a=b+(a-b)$; by \Cref{prop:exactly}, once we condition $a-b \eqs 0$, we have $a=b$.
		\item[{\eqref{ax:cond_init}}]~By \Cref{prop:closedterms}, noting that $c \ll \mathcal N(0,1)$
		\item[{\eqref{ax:fail_incons}}]~By \Cref{prop:closedterms}, because $0 \not \ll 1$
		\item[{\eqref{ax:cong}}]~This follows from \Cref{prop:isomorphic_conditions}, because over $\catname{Aff}$, equivalent scalar equations are nonzero multiples of each other. Still, this is very surprising axiom scheme, which is substantially generalized in \Cref{prop:equivalent_equations}.
	\end{description} 
	%\vspace{-12pt}
\end{proof}

For the remainder of this section, we will show how to use the theory to derive normal forms for conditioning programs.

\begin{proposition}
	\label{prop:elementary}
	Elementary row operations are valid on systems of conditions. In particular, if $S$ is an invertible matrix then
	\[ (A\vec x \eq \vec b)\ret{} \equiv (SA\vec x \eq S\vec b)\ret{} \]
\end{proposition}
\begin{proof}
	Reordering and scaling of equations is \eqref{ax:cond_comm}, \eqref{ax:cong}. For summation, i.e.
	\[ (s \eq t)(u \eq v)\ret{} \equiv (s \eq t)(u + s \eq v + t)\ret{} \]
	instantiate \eqref{ax:cond_subst} with ${(u + x \eq v + t)\ret{}}/{\ret{x}}$. Now use the fact that applying any invertible matrix on the left can be decomposed into elementary row operations.
\end{proof}

\begin{corollary}
	\label{prop:equivalent_equations}
	If $A\vec x = \vec c$ and $B\vec x = \vec d$ are linear systems of equations with the same solution space, then 
	\[ (A\vec x \eq \vec c)\ret{} \equiv (B \vec x \eq \vec d)\ret{} \]
	is derivable. 
\end{corollary}
This generalizes \eqref{ax:cong} to systems of conditions.
\begin{proof}
	If consistent systems are equivalent, then they must be isomorphic by \Cref{prop:affine_equivalence} and we use the previous proposition. If they are inconsistent, we can derive $(0\eq 1)$ and use \eqref{ax:fail_incons},\eqref{ax:fail_absorb} to equate them to $\bot$.
\end{proof}

We give a normal form for closed terms.
\begin{theorem}
	\label{prop:normalization}
	Any closed term can be brought into the form $\nu \vec z. \ret{A\vec z + \vec c}$ or $\bot$. The matrix $AA^T$ is uniquely determined.
\end{theorem}
This is the algebraic analogue of \Cref{prop:closedterms}.
\begin{proof}
	By commutativity, we bring the term into the form
	\[ \nu \vec z. (A \vec z \eq \vec b)\ret{D\vec z+\vec d} \]
	By \Cref{prop:basechange}, we can find invertible matrices $S,T$ such that
	\[ SAT^{-1} = \begin{pmatrix} I_r & 0 \\ 0 & 0 \end{pmatrix} \]
	and $T$ is orthogonal. Using the orthogonal coordinate change $\vec w=T\vec z$ and \Cref{prop:equivalent_equations}, the equations take the form
	\[ \nu \vec w.(SAT^{-1}\vec w \eq S\vec b)\ret{DT^{-1}\vec w + \vec d} \]
	This simplifies to
	\begin{align*}
	\nu \vec w. (\vec w_{1:r} \eq \vec c_{1:r})(0 \eq \vec c_{r+1:n}) \ret{DT^{-1}\vec w + \vec d}
	\end{align*}
	where $\vec c = S\vec b$. We can process the first block of conditions with \eqref{ax:cond_init}. The conditions $(\underline{0} \eq c_i)$ can either be discarded by \eqref{ax:cond_tauto} if $c_i = \underline{0}$ for all $i=r+1,\ldots,n$, or fail by \eqref{ax:fail_incons} otherwise. We arrive at a conditioning-free term.
\end{proof}

\begin{example}
	\[ \nu x.\nu y.(x \eq y) \ret{x,y} \equiv \nu x.\ret{sx,sx} \]
	where $s=1/\sqrt 2$.
\end{example}
\begin{proof}
	We use again the unitary matrix $U$ from \Cref{ex:alg_diagonal}
	\begin{align*}
	\nu x.\nu y.(x \eq y);\ret{x,y}
	&\equiv \nu x.\nu y.(sx + sy \eq -\!sx + sy);\\
	&\quad\quad \ret{sx + sy, -sx + sy} \\
	&\equiv \nu x.\nu y.(x \eq 0)\ret{sx + sy, -sx + sy} \\
	&\equiv \nu y.\ret{sy,sy}
	\end{align*}
	where we apply \eqref{ax:orth}, affine algebra and \eqref{ax:cond_init}.
\end{proof}

Lastly, we give a normal form for conditioning effects: Every effect in $\cond(\gauss)$ can be expressed as $A\vec x \eq \psi$, that is a suitable transformation followed by a soft constraint (\Cref{sec:synth_observe}). However, unlike in a situation where there exists a Frobenius unit, not every effect is of the form $\vec x \eq \psi$ (for example $x_1 - x_2 \eq 0$ is not of that form).

\begin{theorem}[Normal forms]
	\label{prop:normalform_uniqueness}
	Every term $\vec x : \rv^n \vdash u : \rv^0$ can either be brought into the form $\bot$ or
	\begin{equation} \nu \vec z.A \vec x \eq B\vec z + \vec c \label{eq:normalform} \end{equation}
	where $A \in \R^{r \times n}$ is in reduced echelon form with no zero rows. The values of $A$, $\vec c$ and $BB^T$ are uniquely determined.
\end{theorem}
\begin{proof}
	Through the commutativity axioms, we can bring $u$ into the form $\nu \vec z.A \vec x \eq B\vec z + \vec c$	for some general $A$. Find an invertible matrix $S$ that turns $A$ into reduced row echelon form, and apply it to the condition via \Cref{prop:elementary}. The zero columns don't involve $\vec x$, so we use \Cref{prop:normalization} to evaluate the condition involving $\vec z$ separately. We either obtain $\bot$ or the desired form \eqref{eq:normalform}. For uniqueness, we consider the term's denotation $(A\vec x \eq \eta) : n \obsto 0$ in $\cond(\gauss)$, where $\eta = \mathcal N(\vec c,BB^T)$. We must show that $A$ and $\eta$ can be reconstructed from the observational behavior of the denotation. The proof is given in the appendix (\Cref{prop:uniqueness_proof}).
\end{proof}

==> intro.tex <==
\section{Introduction}\label{sec:intro} \lstset{style=python_ppl}

Probabilistic programming is a programming paradigm that uses code to formulate generative statistical models and perform inference on them~\cite{van_de_meent:ppl_introduction, probmods2}. Techniques from programming language theory can be used to understand modelling assumptions such as conditional independence, as well as enable optimizations that improve the efficiency of various inference algorithms. 

%In \cite{staton:commutative_semantics}, three central constructs have been identified for probabilistic programming languages: \lstinline|sample|, \lstinline|observe| and \lstinline|normalize|.
As an example problem, we shall consider a noisy measurement: Our \emph{prior} assumption about the distribution of some quantity $X$ is that it is normally distributed with mean $\mu=50$ and standard deviation $\sigma=10$. We only have access to a noisy measurement $Y$, which itself has standard deviation $5$, and observe a value of $Y=40$. Conditioned on that observation, the \emph{posterior} distribution over $X$ is now $\N(42,\sigma)$ with $\sigma = \sqrt{20} \approx 4.47$. 

There are two different ways of expressing the conditioning on an observation in code: \emph{scoring} and \emph{exact conditioning}. While the idea of exact conditioning is not novel, the goal of this article is to rigorously spell out this paradigm, give semantics to it and analyze its properties. 

To recap, under \emph{scoring}, we understand a construct like \lstinline|score| or \lstinline|observe| which records a likelihood to re-weight the current execution trace of the probabilistic program. A scoring implementation of the noisy measurement example looks like this
\begin{lstlisting}
x = normal(50, 10)  # prior
observe(40, normal(x,5))  # observation
\end{lstlisting}
The idea of Monte Carlo simulation is to run the program many times, picking different values for \lstinline|x| from the normal distribution. The \lstinline|observe| command in this example weights the execution trace with the density function of the distribution $\N(x,5)$ evaluated at $40$. This makes execution traces more likely whose value of \mlstinline|x| lies closer to $40$.
Scoring constructs like \lstinline|observe| are widely available in popular probabilistic languages such as \textsc{Stan} \citep{stan} or \textsc{WebPPL} \citep{dippl}.\\
%Scoring with likelihoods from $\{0,1\}$ is sometimes called a \emph{hard constraint}, as opposed to more general \emph{soft constraints}. The prototypical way of performing inference on scoring programs is by likelihood-weighted importance sampling. Hard constraints turn this into mere rejection sampling, because likelihood-zero traces are discarded entirely. Replacing hard constraints by equivalent soft ones can thus be beneficial for inference efficiency. \\

We contrast scoring with \emph{exact conditioning}, which features a construct here denoted $E_1 \eq E_2$ expressing that $E_1$ and $E_2$ shall be conditioned to be exactly equal. The noisy measurement formulated using exact conditioning reads
\begin{lstlisting}
x = normal(50,10) # prior
y = normal(x,5)    # measurement
y =:= 40           # exact observation
\end{lstlisting}

Exact conditions are strictly more powerful than scoring, because we can express \lstinline|observe(x,D)| in terms of conditioning on a freshly generated sample as \lstinline|let y = sample(D) in y =:= x|. On the other hand, not every exact conditioning program can be expressed in terms of scoring. For \emph{discrete probability}, there is no problem, and we can express an exact condition $E_1 \eq E_2$ by the hard constraint \lstinline|observe($E_1$, dirac($E_2$))|, where \lstinline|dirac| is the Dirac distribution\todo{S: I replaced score with a dirac constraint, is that ok?}. This causes an execution trace to be discarded if the condition is not met. This encoding is no longer viable for continuous distributions such as Gaussians: For example, the program
\begin{lstlisting}
x = normal(0,1); x =:= 40
\end{lstlisting}
should return \lstinline|x=40| deterministically, because $x$ is conditioned to have that value. On the other hand, the attempted program with a score-based hard constraint
\begin{lstlisting}
x = normal(0,1); observe(x, dirac(40))
\end{lstlisting}
will reject every execution trace, because the probability that \lstinline|x==40| is true equals zero. 

Variants of exact conditioning are available in different frameworks; in \textsc{Hakaru} \citep{shan_ramsey}, certain exact conditioning queries can be addressed using symbolic disintegration, but $(\eq)$ is not a first-class construct in Hakaru. \textsc{Infer.NET} \citep{InferNET18} does allow exact conditioning on variables and employs an approximate inference algorithm to solve the resulting queries (e.g. \citep{infernet_tutorial}). \\

We will consider two settings as central examples, namely
\begin{enumerate}
	\item \emph{finite probability}, that is finite sets and discrete distributions
	\item \emph{Gaussian probability}, that is affine-linear maps and multivariate normal noise. 
\end{enumerate}
\todo[inline]{Is this supposed to be a summary of the paper? If so, add cross references. But there are other summaries of the paper in this intro. We should perhaps have an outline of what is coming in the intro.}
We give a unified account of discrete and continuous probability using the formalism of Markov categories. Desirable properties of exact conditioning such as the ability to reorder conditions can be established purely abstractly. Our type-theoretic approach to conditioning will also help addressing counterintuitive behavior such as Borel's paradox. 

\subsection{Compositional Reasoning about Exact Conditions}

\lstset{style=python_ppl}

We'll briefly discus some advantages of the exact conditioning paradigm using the informal Python-like language for Gaussian probability from before. As a case study, this language will be formalized in \Cref{sec:gaussian_language}, and a Python implementation for it is available under \cite{gaussianinfer}. While the Gaussian setting is certainly restrictive, it already emphasizes the difficulties of working with continuous probability distributions, and it is expressive enough to express a range of interesting applications such as ridge regression, Kalman filters and Gaussian processes (``kriging''). Our results and methodology however are general and not tied to the specific example of Gaussian probability. The advantages of exact conditioning we propose are:

\begin{enumerate}
\item Exact conditioning is intuitive to use and allows the programmer to cleanly decouple the generative model from the data observation stage.
\item Exact conditioning lends itself to logical reasoning about programs. For example, after conditioning $s \eq t$, the expressions $s$ and $t$ are known to be equal and can be interchanged \eqref{eqn:substlong}. 
\item Exact conditioning enjoys good formal properties (e.g. \eqref{eqn:initcommutativity}, \eqref{eqn:initlong}) which allow us to simplify programs compositionally.
\end{enumerate}

To elaborate these points, we consider the example of a simple Gaussian random walk with 100 steps, together with a table \lstinline|obs| of exact observations (\Cref{fig:rw}). A straightforward implementation would be to first generate the entire random walk, and then condition on the observations
\begin{lstlisting}
# generative model
for i in range(1,100):
  y[i] = y[i-1] + normal(0,1)
# observations
for j in obs:
  y[j] =:= obs[j]
\end{lstlisting}

The same program is more complicated to express without exact conditioning: Using soft conditions, the observations would need to be known at the time of generation and \lstinline|observe| commands need to be issued in-place, breaking the decoupling between the model and the data. 

On the other hand, rewriting the original model in such a way may improve the efficiency of inference. We can verify such a transformation using compositional reasoning: As we will show, it is consistent to reorder program lines as long as the dataflow is respected \eqref{eqn:initcommutativity}, so the random walk program is equivalent to the following version with interleaved observations
\begin{lstlisting}
for i in range(1,100):
  y[i] = y[i-1] + normal(0,1)
  if i in obs: y[i] =:= obs[i]
\end{lstlisting}
In the observation branch, we can now use initialization principle \eqref{eqn:initlong} to set \lstinline|y[i]| to its target value directly as \lstinline|y[i] = obs[i]|. The remaining condition becomes \lstinline|(y[i] - y[i-1]) =:= normal(0,1)| so we obtain 
\begin{lstlisting}
for i in range(1,100):
  if i in obs:
    y[i] = obs[i]
    (y[i] - y[i-1]) =:= normal(0,1) 
  else:
    y[i] = y[i-1] + normal(0,1)
\end{lstlisting}
In this version of the program, all exact conditions can now be replaced by \lstinline|observe| statements:
\begin{lstlisting}
for i in range(1,100):
  if i in obs:
    y[i] = obs[i]
    observe(y[i] - y[i-1] , normal(0,1))
  else:
    y[i] = y[i-1] + normal(0,1)
\end{lstlisting}
We can run this resulting program directly using a Monte Carlo simulation in Stan or WebPPL. \\

\begin{figure}[h]
	\centering
	\includegraphics[width=0.40\textwidth]{conditioning/rw_raw.png}
	\includegraphics[width=0.40\textwidth]{conditioning/rw_conditioned.png}
	\caption{Gaussian random walk (left) and conditioned posterior (right) with four exact observations at $i=20,40,60,80$\label{fig:rw}}
\end{figure}

In \Cref{sec:gaussian_language}, we formalize the operational semantics of our Gaussian language, in which there are two key commands: drawing from a standard normal distribution ($\normal()$) and exact conditioning $(\eq)$. The operational semantics is defined in terms of configurations $(t,\psi)$ where $t$ is a program and $\psi$ is a state, which here is a Gaussian distribution. Each call to $\normal()$ introduces a new dimension into the state~$\psi$, and conditioning $(\eq)$ alters the state~$\psi$, using a canonical form of conditioning for Gaussian distributions (\Cref{sec:recap_gauss}).

In our first version of the random walk example, the operational semantics will first build up the prior distribution shown on the left in \Cref{fig:rw}, and then the second part of the program will condition to yield a distribution as shown on the right. But for the other programs above, the conditioning will be interleaved in the building of the model.\\

In stateful programming languages, composition of programs is often complicated and local transformations are difficult to reason about. However, we will show that for the Gaussian language, compositionality and local reasoning remain straightforward. Throughout this section we have used several program transformations to compositional illustrate reasoning about exact conditioning. Abstractly, we have used the following properties, which are valid, as we will show in this paper:
\begin{itemize}
	\item Program lines can be reordered as long as dataflow is respected. That is, the \emph{commutativity equation} remains valid for programs with conditioning
	\begin{equation}
	\begin{array}{l}
	\letin x u \\
	\letin y v t
	\end{array}
	\equiv
	\begin{array}{l}
	\letin y v \\
	\letin x u t
	\end{array} \label{eqn:initcommutativity}
	\end{equation}
	where $x$ not free in $v$ and $y$ not free in $u$.
	\item We have a \emph{substitution law}: if $t\eq u$ appears in a program, then later occurrences of $t$ may be replaced by $u$.
	\begin{equation}(t\eq u);v[t/x]\quad \equiv
	\quad (t\eq u);v[u/x]
	\label{eqn:substlong}
	\end{equation}
	\item As a special base case, if we condition a normal variable on a constant $\underline c$, then that variable is \emph{initialized} to this value
	\begin{equation}\letin x {\normal()} {(x\eq \underline c);t} \quad \equiv
	\quad t[\underline c/x]
	\label{eqn:initlong}
	\end{equation}
\end{itemize}

\subsection{Denotational Semantics: The Cond Construction}

No style of probabilistic modelling is immune to fallacies and paradoxes. Exact conditioning is indeed sensitive in this regard (\Cref{sec:paradoxes}), and so it is important to show that where it is used, it is consistent in a compositional way. While scoring has straightforward measure-theoretic semantics, describing the intended meaning of exact conditioning is more complex. Making this precise is one of the goals of this article.  

Purely probabilistic computation (without conditioning) between finite sets can be described semantically using stochastic matrices. Inference computation (with conditioning) on the other hand is commonly described by \emph{sub}stochastic matrices, where the probabilities do not sum to $1$ because of rejected outcomes. In the Gaussian setting, a probabilistic computation can be concisely described by a matrix $A$ and the mean and covariance $(\mu,\Sigma)$ of the Gaussian noise. A contribution of this paper is to identify an appropriate analogue of substochastic matrices in this Gaussian setting. \\

We solve this by developing a systematic account of the extension of probabilistic computation to inference computation. A notion of probabilistic computation is supplied abstractly in the form of a Markov category $\C$ (\Cref{sec:synth_conditioning}). We develop a general theory of conditioning and inference problems for such categories in (\Cref{sec:inferenceproblems}). The $\cond$ construction \Cref{sec:cond} is then a means to faithfully extend the Markov category $\C$ by morphisms $(\eqo k_0)$ which make exact observations a first-class (internal) notion.
Intuitively, a morphism $X \obsto Y$ in $\cond(\C)$ is a contextual equivalence class of an open program of the form
\[ x : X \vdash \letin {(y,k)} {f(x)} {(k \eqo k_0); y} \]
These are normal forms for straight-line inference computation. The correspondence between open programs and categorical morphisms is made canonical using the notion of \emph{internal language} of a Markov category. Under this, Markov categories correspond precisely to a class of first-order probabilistic programming languages.

Our use of Markov categories is agnostic to whether finite or continuous probability is being used. We can derive desirable properties of exact conditioning in this purely abstract setting. Notably, measure-theory, densities and limits are completely absent from our analysis. Instead, we rely on dataflow properties which are natural from a programming point of view. 
The convenient formalism of string diagrams (\Cref{sec:synth_conditioning}) serves as a concise alternative syntax for program equations, as well as allowing us to make connections with graphical models and derive a graphical language for conditioning.

\subsection{Outline}

In order to introduce and study the exact conditioning paradigm, we introduce two example languages with an exact conditioning construct. A language $\ppi$ for finite probability (\Cref{sec:finstoch}) and the Gaussian language. Semantics of $\ppi$ is standard, but semantics of the Gaussian language is new. We define an observational semantics for the Gaussian language in \Cref{sec:gaussian_language} and a denotational one in \Cref{sec:denotational}, which we prove fully abstract (\Cref{prop:full_abstraction}).

Abstracting away from these particular examples, we develop a general framework for exact conditioning. We begin by showing a correspondence between a class of first-order probabilistic programming languages and mathematical structures called Markov and CD- categories (\Cref{sec:cd_cats}). At the heart of this correspondence is the CD-calculus, which is the internal language of CD categories \Cref{sec:cd-calc}. We recall categorical definitions of probabilistic concepts such as determinism, independence and conditioning and give an abstract account of inference problems in \Cref{sec:abstract_cond}.

The core contribution of this article is the $\cond$ construction (\Cref{sec:cond}), which extends a Markov category with effects $X \to I$ for exact observations. On the programming language side, this corresponds to adding an exact observation construct $(\eqo)$ to the language. The $\cond$ construction requires no measure theory, densities or limits. It is instead closely tied to reasoning in terms of program transformations. Indeed the Cond construction can be understood as giving normal forms for straight-line programs with exact observations, modulo contextual equivalence. 

In \Cref{sec:finstoch}, we leave the generality of Markov categories and analyze the $\cond$ construction applied to our two main examples, finite and Gaussian probability. This means studying the contextual equivalence of straight-line conditioning programs:

We show that the $\cond$ construction applied to finite probability describes substochastic kernels modulo automatic renormalization (\Cref{sec:finprojstoch}). This fully characterizes contextual equivalence for straight-line inference with discrete probability, and refines the semantics using the subdistribution monad. Our discussion shows interesting connections between the admissibility of automatic normalization and the availability of branching in probabilistic programs (\Cref{sec:straightline}). A full characterization of the $\cond$ construction applied to Gaussian probability is future work, though we gave a sound algebraic theory in \cite{2021compositional}.


\paragraph{Note} The starting points for this article are our paper in the Proceedings of LICS 2021~\cite{2021compositional} and the first author's DPhil thesis~\cite{dariothesis}. We expose the Cond construction in a detailed and self-contained manner with emphasis on program equations and contextual equivalence. The characterizations in \Cref{sec:finstoch} and the recognition of the special role of branching in \Cref{sec:straightline} are novel.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

